Fusing CNNs and statistical indicators to improve image classification

Convolutional Networks have dominated the field of computer vision for the last ten years, exhibiting extremely powerful feature extraction capabilities and outstanding classification performance. The main strategy to prolong this trend relies on further upscaling networks in size. However, costs increase rapidly while performance improvements may be marginal. We hypothesise that adding heterogeneous sources of information may be more cost-effective to a CNN than building a bigger network. In this paper, an ensemble method is proposed for accurate image classification, fusing automatically detected features through Convolutional Neural Network architectures with a set of manually defined statistical indicators. Through a combination of the predictions of a CNN and a secondary classifier trained on statistical features, better classification performance can be cheaply achieved. We test multiple learning algorithms and CNN architectures on a diverse number of datasets to validate our proposal, making public all our code and data via GitHub. According to our results, the inclusion of additional indicators and an ensemble classification approach helps to increase the performance in 8 of 9 datasets, with a remarkable increase of more than 10% precision in two of them.

==> table_cnns_old.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htpb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{2}{c}{\textbf{DenseNet201}} & \multicolumn{2}{c}{\textbf{Inception ResNet V2}} & \multicolumn{2}{c}{\textbf{Inception V3}} & \multicolumn{2}{c}{\textbf{VGG19}} & \multicolumn{2}{c}{\textbf{Xception V1}} \\ \cline{2-11} 
\multicolumn{1}{c}{} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} & \textbf{Mean} & \textbf{Std.} \\ \hline
\textbf{Cars 196} & 75.46\% & 2.74\% & \textbf{75.80\%} & \textbf{1.26\%} & 69.00\% & 7.18\% & 0.00\% & 0.00\% & 65.42\% & 1.51\% \\
\textbf{Caltech birds2011} & 66.60\% & 0.67\% & \textbf{67.95\%} & \textbf{0.88\%} & 61.81\% & 0.47\% & 5.16\% & 12.63\% & 62.23\% & 0.56\% \\
\textbf{Cats vs dogs} & 98.71\% & 0.14\% & \textbf{99.01\%} & \textbf{0.02\%} & 98.93\% & 0.16\% & 97.97\% & 0.32\% & 98.80\% & 0.10\% \\
\textbf{Citrus leaves} & 72.59\% & 10.04\% & 88.15\% & 2.53\% & 87.48\% & 1.08\% & \textbf{93.88\%} & \textbf{0.65\%} & 81.72\% & 0.59\% \\
%\textbf{Clouds} & 70.56\% & 0.00\% & \textbf{92.74\%} & \textbf{1.06\%} & 92.23\% & 2.05\% & 91.31\% & 1.62\% & 1.27\% & 0.00\% \\
\textbf{Deep weeds} & 49.67\% & 16.66\% & 91.02\% & 0.44\% & 90.51\% & 0.33\% & \textbf{91.89\%} & \textbf{1.32\%} & 64.52\% & 6.48\% \\
\textbf{Malaria} & 85.88\% & 0.66\% & \textbf{97.09\%} & \textbf{0.10\%} & \textbf{97.09\%} & \textbf{0.04\%} & 96.16\% & 0.11\% & 87.60\% & 1.66\% \\
\textbf{Oxford flowers102} & \textbf{82.39\%} & \textbf{0.57\%} & 77.70\% & 0.70\% & 68.59\% & 1.23\% & 6.74\% & 9.20\% & 76.25\% & 0.44\% \\
\textbf{Plant leaves} & 74.93\% & 2.39\% & \textbf{95.78\%} & \textbf{0.89\%} & 94.13\% & 0.88\% & 93.00\% & 0.69\% & 71.05\% & 1.11\% \\
\textbf{Plant village} & 86.76\% & 3.00\% & \textbf{99.54\%} & \textbf{0.07\%} & 99.29\% & 0.07\% & 99.24\% & 0.28\% & 92.49\% & 0.62\% \\ \hline
\end{tabular}%
}
\caption{Results of different CNN architectures. All values indicate the macro average weighted precision.}
\label{tab:cnn_results}
\end{table*}

==> table_final_comparison.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Final comparison
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[htpb]
\centering
\resizebox{1\linewidth}{!}{%
\begin{tabularx}{\textwidth}{@{}ccccccc@{}}
\toprule
\textbf{Dataset} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Individual CNN\\ Best result\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Best classification\\ with statistical\\ features\end{tabular}}} & \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Best classification\\ CNN + Best classification\\ with statistical features\end{tabular}}} \\ \midrule
\textbf{Cars 196} & Densenet201 & 78.44\% & RF & 3.95\% & Inception V3 + SVM-poly & \textbf{88.63\%} \\

\textbf{Caltech birds2011} & Inception ResNet V2 & 69.10\% & RF & 3.66\% & Inc. Resnet V2 + RF & \textbf{72.18\%} \\

\textbf{Cats vs dogs} &  ResNet V2 & 99.00\% & LDA & 63.51\% & Inc. Resnet V2 + Avg & \textbf{99.03}\% \\

\textbf{Citrus leaves} & VGG19 & 93.80\% & LDA & 89.41\% & VGG19 + Avg & \textbf{95.45}\% \\

%\textbf{Clouds} & Inception ResNet V2 & 93.40\% & RF & 90.12\% & Inc. ResNet V2 + SVM-sig & \textbf{95.05\%} \\

\textbf{Deep weeds} & VGG-19 & 93.14\% & RF & 68.74\% & VGG19 + KNN & 92.90\% \\

\textbf{Malaria} & Inception ResNet V2 & 97.20\% & RF & 95.86\% & Inception V3 + Avg & \textbf{97.30\%} \\

\textbf{Oxford flowers102} & DenseNet201 & 82.91\% & LDA & 33.19\% & Densenet201 + SVM-poly & \textbf{96.23\%} \\

\textbf{Plant leaves} & Inception ResNet V2 & 96.58\% & LDA & 81.98\% & Inc. ResNet V2 + KNN & \textbf{96.77\%} \\

\textbf{Plant village} & VGG19 & 99.60\% & RF & 80.32\% & Inc. Res. V2 + LR/KNN/SVM & \textbf{99.69\%} \\ \bottomrule
\end{tabularx}%
}
\caption{Comparison of (a) result of the best CNN model, (b) best classification achieved with statistical features and ML classifiers and (c) results of the best combination between the probabilities of the best classifier trained with statistical features and the output probabilities of the CNN. All values indicate the macro average weighted precision.}
\label{tab:results_comparison}
\end{table*}


==> table_results_combination_old.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htpb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabularx}{1.15\textwidth}{@{}lYYYYYYYY@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} & \multicolumn{8}{c}{\textbf{CNN output probabilities + Best model with statistical features}} \\ \cmidrule(l){2-9} 
\multicolumn{1}{c}{} & \textbf{Average} & \textbf{\begin{tabular}[c]{@{}c@{}}Logistic\\ Regression\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Linear\\ Discriminant\\ Analysis\end{tabular}} & \textbf{KNN} & \textbf{\begin{tabular}[c]{@{}c@{}}SVM\\ poly\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SVM\\ rbf\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SVM\\ sigmoid\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Random\\ Forest\end{tabular}} \\ \midrule
\textbf{Cars 196} & 73.94\% & 73.94\% & 72.90\% & 74.21\% & \textbf{87.29\%} & 75.36\% & 74.14\% & 77.93\% \\
\textbf{Caltech birds2011} & 68.89\% & 68.91\% & 69.25\% & 68.90\% & \textbf{73.15\%} & 68.89\% & 68.91\% & 72.65\% \\
\textbf{Cats vs dogs} & \textbf{99.03\%} & \textbf{99.03\%} & \textbf{99.03\%} & \textbf{99.03\%} & \textbf{99.03\%} & \textbf{99.03\%} & \textbf{99.03\%} & \textbf{99.03\%} \\
\textbf{Citrus leaves} & \textbf{92.06\%} & 89.46\% & 86.81\% & 87.89\% & 88.68\% & 87.89\% & 86.81\% & 85.97\% \\
\textbf{Clouds} & 94.07\% & 94.72\% & 94.08\% & 93.89\% & 92.23\% & 94.29\% & \textbf{95.05}\% & 92.96\% \\
\textbf{Deep weeds} & 92.64\% & 92.73\% & 92.59\% & \textbf{92.87\%} & 92.43\% & 92.78\% & \textbf{92.87\%} & 86.53\% \\
\textbf{Malaria} & \textbf{97.24\%} & 97.18\% & 97.13\% & 97.20\% & 97.13\% & 97.16\% & 97.22\% & 97.16\% \\
\textbf{Oxford flowers102} & 53.92\% & 67.52\% & 89.33\% & 65.05\% & \textbf{93.01\%} & 71.44\% & 72.09\% & 88.81\% \\
\textbf{Plant leaves} & \textbf{94.41\%} & 93.91\% & 93.83\% & 94.05\% & 93.84\% & 93.81\% & 93.92\% & 93.80\% \\
\textbf{Plant village} & \textbf{99.53\%} & \textbf{99.53\%} & \textbf{99.53\%} & \textbf{99.53\%} & \textbf{99.53\%} & \textbf{99.53\%} & \textbf{99.53\%} & 97.13\% \\ \bottomrule
\end{tabularx}%
}
\caption{Results achieved combining the class probabilities from the best CNN model and the class probabilities from the best classifier trained on statistical features. The average is also considered. All values are expressed in terms of macro average weighted precision.}
\label{tab:results_combination}
\end{table*}
